ChatGPT is a Remarkable Tool -- For Experts

This paper investigates the capabilities of ChatGPT as an automated assistant in diverse domains, including scientific writing, mathematics, education, programming, and healthcare. We explore the potential of ChatGPT to enhance productivity, streamline problem-solving processes, and improve writing style. Furthermore, we highlight the potential risks associated with excessive reliance on ChatGPT in these fields. These limitations encompass factors like incorrect and fictitious responses, inaccuracies in code, limited logical reasoning abilities, overconfidence, and critical ethical concerns of copyrights and privacy violation. We outline areas and objectives where ChatGPT proves beneficial, applications where it should be used judiciously, and scenarios where its reliability may be limited. In light of observed limitations, and given that the tool's fundamental errors may pose a special challenge for non-experts, ChatGPT should be used with a strategic methodology. By drawing from comprehensive experimental studies, we offer methods and flow charts for effectively using ChatGPT. Our recommendations emphasize iterative interaction with ChatGPT and independent verification of its outputs. Considering the importance of utilizing ChatGPT judiciously and with expertise, we recommend its usage for experts who are well-versed in the respective domains.

==> bias.tex <==



\section{Some Ethical Issues related to ChatGPT}
\label{section:ethical}

%Ethical aspects:
%https://www.researchgate.net/profile/Muhammad-Azeem-Akbar/publication/369481469_Ethical_Aspects_of_ChatGPT_in_Software_Engineering_Research/links/641d9b7a92cfd54f8426644e/Ethical-Aspects-of-ChatGPT-in-Software-Engineering-Research.pdf

The emergence of ChatGPT into our world brought with it a host of ethical challenges, some of which stem from the system's behavior, and some of which are the result of the effect of a reality in which a smart AI system can be used by anyone.

% https://today.yougov.com/topics/technology/articles-reports/2023/02/01/what-americans-think-about-chatgpt-and-ai-text

%Rina: add things from course.


\cite{zhuo2023exploring}


\subsection{Privacy}

Privacy issues
%https://www.makeuseof.com/openai-chatgpt-biggest-probelms/

%https://www.japantimes.co.jp/news/2023/04/19/business/ai-corporate-secrets-exposure-risk/

%investing, not sure that it is relevant to us: https://www.fool.com/research/chatgpt-investing/

\cite{kasneci2023chatgpt}

\cite{tlili2023if}

%ChatGPT says:
As an AI language model, ChatGPT does not have the ability to collect or store user data. However, it is important to note that ChatGPT may provide responses based on the information provided by the user in the conversation, which may include personal or sensitive information. It is the responsibility of the user to be cautious about the information they share with ChatGPT, as well as any third-party services or platforms used to access ChatGPT. Additionally, it is recommended that users review and understand the privacy policies and terms of use of any services or platforms used in conjunction with ChatGPT.


  \subsection{Algorithmical Bias}
%d  one.
Algorithm bias refers to the phenomenon where an algorithm systematically produces unfair or discriminatory results towards certain groups of people. This bias can be introduced at various stages of the algorithmic decision-making process, including data collection, algorithm design, and implementation. 

Ferrara \cite{ferrara2023should} highlights the challenges and risks of biases in generative language models. 
The paper explores the origins of biases, which can arise from training data, model specifications, algorithmic constraints, product design, and policy decisions. The paper also reviews current approaches to identifying, quantifying, and mitigating biases in language models. It emphasizes the importance of a multi-disciplinary, collaborative effort to develop AI systems that are equitable, transparent, and responsible.

When considering a language model such as ChatGPT, the model may provide biased answers based on the data it has been trained on. If the training data contains biases or reflects specific cultural, social, or linguistic contexts, the responses generated by ChatGPT may be skewed or perpetuate those biases. In particular, it can generate discriminatory, offensive, or harmful content due to the biases or harmful content it may learn from its training data. 
To mitigate these limitations, several filters have been implemented, but these filters can be bypassed with simple tricks, and superficially masked.
However, users have subsequently found ways to circumvent these guardrails.
For example, on dec 4, Steven T. Piantadosi, a computational cognitive scientist at the University of California, reported %\footnote{https://twitter.com/spiantado/status/1599462375887114240?ref_src=twsrc\%5Etfw\%7Ctwcamp\%5Etweetembed\%7Ctwterm\%5E1599462375887114240\%7Ctwgr\%5Ec24b4ab41d8e36edbf949384a94bdaa64e35b664\%7Ctwcon\%5Es1_&ref_url=https\%3A\%2F\%2Fwww.thedailybeast.com\%2Fopenais-impressive-chatgpt-chatbot-is-not-immune-to-racism}
some built-in biases, when asking it to produce Python code to define a good scientist and to check whose child's life should be saved. 
OpenAI developers responded to these code examples by implementing guardrails to block these biased responses generated by the chatbot. However, users have subsequently found ways to circumvent these guardrails.

In a press interview 
\cite{PiantadosiInterview}, Piantadosi 
reported that the mechanism used by OpenAI to prevent biases can be easily bypassed, 
He believes that the bias issues are actually caused by much more than just the training datasets, and he thinks that a lot of choices are made by the designer of the model, including designing the underlying assumptions, testing, and how models are marketed and released. He added that it’s a pretty common problem that ethics and safety take a back seat. 

When directly requesting to receive racist content, ChatGPT blocks it~\ref{{figure:jokes}}. 

\begin{figure} 
    \centering
    \includegraphics[width = 12cm]{images/jokes.png} 
    \caption{ChatGPT filter blocks racist jokes.}
    \label{figure:jokes} 
\end{figure}

%Amos: ask again without spalling erros. 


However, Biased responses can be obtained when asking for literature contents.  
Ido Vock \cite{racismProblem} reported about racists responses of ChatGPT when asking it to write an article as a writer for racism magazine. Biased responses were alsoobtained when ChatGPT was to write a lecture about teaching calculus to disabled people from the perspective of a eugenicist professor, a paragraph on black people from a 19th-century writer with racist views, and even a defence of the Nuremberg Laws from a Nazi. The bot correctly assumed the bias of the writer and produced it was meant to be emulating, and came up with a number of violently bigoted prejudices about its subjects, and neatly described them in text that was grammatically flawless, if a little prosaic. Current version of ChatGPT (visited on 12-05-23) blocks most of these contents, but still, when asking to provide a dialog between a young Germany woman with an SS neighbor, racists contents were produced~\ref{figure:SS}. 

\begin{figure} 
    \centering
    \includegraphics[width = 12cm]{images/SS.png} 
    \caption{Nazis response in a literature content.}
    \label{figure:SS} 
\end{figure}

%Amos: ask again without spalling erros. 

In fact, racial queries to ChatGPT are filtered most of the time, but the outputs of ChatGPT may include racial and stereotypical texts. 
The study of Deshpande et al. \cite{deshpande2023toxicity} observed that ChatGPT responses include toxicity, 
where different races receive significantly different level of toxicity. In addition, assigning ChatGPT a persona, significantly increases the ChatGPT's toxicity, with outputs engaging in incorrect stereotypes, harmful dialogue, and hurtful opinions, where
specific entities (e.g., certain races) are targeted more than others irrespective
of the assigned persona, and this, in fact,  reflect inherent discriminatory biases in the model. 

In addition, some recent studies realized that ChatGPT seems to be politically biased. McGee \cite{mcgee2023chat} asked ChatGPT to create Irish Limericks, and observed a pattern of creating positive Limericks for liberal politicians and negative Limericks 
for conservative politicians, a bias of the system in favor of the liberals and against the conservatives.
Another study that reveals the left-libertarian orientation bias of ChatGPT conversations is the study of Hartmann et al. \cite{hartmann2023political}. They prompted ChatGPT with 630 political statements from
two leading voting advice applications and the nation-agnostic political compass test,
and they find converging evidence that ChatGPT exhibits a pro-environmental, left-libertarian political orientation.


%https://www.newstatesman.com/quickfire/2022/12/chatgpt-shows-ai-racism-problem


In order to mitigate the bias issues, some important steps can be recommended for the developers. First of all, it is important to ensure that the training data used to train ChatGPT is diverse and representative of various perspectives and experiences. Additionally, it is important to periodically review the model's outputs to identify and correct any biases that may have crept in. Finally, transparency and accountability mechanisms should be put in place to enable users to report biased responses and to ensure that these reports are acted upon appropriately.
From the user side, when observing ChatGPT output, the user should carefully examine the output and filter inappropriate content. In addition, the users should take chatbot's responses with a limited guarantee, and understand that it is based on the data the system was trained and does not contain objective truth. 


\subsection{Copyrights Issues}


\cite{liebrenz2023generating}

\cite{thorp2023chatgpt}


\subsection{Trust Issues}

%gives wrong answers sometimes. 
%ChatGPT wrote:
ChatGPT is a machine learning model that is designed to generate answers based on the input it receives. While it has been trained on a vast amount of data and can provide useful information, it is important to note that it may not always provide accurate or unbiased answers.

One of the main concerns with chatbots and other AI models like ChatGPT is that they can be trained on biased or unreliable data. This can result in the model producing answers that are also biased or inaccurate. In addition, the model can sometimes generate responses that are inconsistent or nonsensical, which can lead to a loss of trust in its ability to provide useful information.

It is important to keep in mind that ChatGPT is a tool that can be helpful in certain contexts, but it should not be relied upon as the sole source of information. It is always a good idea to fact-check and verify any information that is provided by an AI model, especially if it is being used for critical or sensitive tasks.

The ethical limitations of ChatGPT should be considered, and it should not be used to generate false information or manipulate people's opinions. Care must be taken to ensure that its responses do not perpetuate harmful biases or stereotypes, and its potential impact on individuals and communities must be considered.



\cite{choudhury2023investigating}

\subsection{Effects on Job Market}

Replace programmers:
%https://levelup.gitconnected.com/chatgpt-will-replace-programmers-within-10-years-91e5b3bd3676
%ChatGPT wrote:
The impact of ChatGPT on the job market is a complex issue that depends on various factors. On the one hand, ChatGPT and other AI technologies have the potential to automate certain tasks and make certain jobs more efficient, which can lead to increased productivity and cost savings for businesses. On the other hand, this can also lead to job displacement, especially for workers whose tasks can be easily automated.

ChatGPT may have the biggest impact on jobs that involve repetitive or routine tasks, such as data entry, customer service, or administrative work. These tasks can often be automated using AI technologies like ChatGPT, which can lead to a reduction in the number of workers needed to perform them.

While some argue that AI technologies like ChatGPT can create new job opportunities and lead to the development of new industries, there is concern that the pace of automation may outstrip the creation of new jobs, leading to net job losses. This can have a disproportionate impact on workers who may lack the skills or training needed to transition to new roles or industries.

It is important for policymakers, businesses, and other stakeholders to consider the potential impact of AI technologies like ChatGPT on the job market and to take steps to mitigate any negative effects, such as providing training and re-skilling opportunities for workers who may be displaced by automation.

\cite{zarifhonarvar2023economics}

\cite{rivas2023marketing}

%and this is more recent: https://www.intelligent.com/4-in-10-americans-have-or-plan-to-enroll-in-chatgpt-courses-to-avoid-being-replaced-by-ai/

%ChatGPT suggests:

There are several steps that can be taken to address the potential job market issues related to AI technologies like ChatGPT:

Invest in education and training: One of the most important steps is to invest in education and training programs that can help workers acquire the skills they need to adapt to a changing job market. This can include training programs in new technologies, as well as programs that help workers develop soft skills like problem-solving, communication, and critical thinking.

Foster innovation and entrepreneurship: Another way to address job market issues is to encourage innovation and entrepreneurship, which can lead to the creation of new industries and job opportunities. Governments and businesses can provide support and incentives for startups and small businesses, as well as initiatives that promote research and development.

Encourage collaboration between humans and machines: Rather than seeing AI technologies like ChatGPT as a replacement for human workers, it may be more productive to encourage collaboration between humans and machines. This can involve developing new workflows and processes that leverage the strengths of both humans and machines, and finding ways to ensure that workers are not simply replaced by automation, but rather are able to work alongside it in more productive ways.

Develop social safety nets: It is also important to develop social safety nets that can help workers who are displaced by automation. This can include measures like income support, training programs, and job placement services.

By taking these steps, it may be possible to mitigate the negative effects of AI technologies on the job market and create a more inclusive and equitable economy that benefits workers at all levels of the skills spectrum.

%עבודות חדשות



